Semi-Decentralized Multi-Spacecraft Collision Avoidance under Communication Constraints

Current spacecraft collision-avoidance operations rely on intermittent ground-station contacts, requiring operators to plan with delayed and asynchronously updated information. Consequently, maneuvers must be planned with only intermittent information sharing between operators, raising the question of how much coordination is needed to achieve collision-avoidance performance comparable to centralized planning. Although decision-theoretic approaches such as partially observable Markov decision processes (POMDPs) capture the sequential and uncertain nature of collision avoidance, existing multiagent extensions typically assume either continuous information sharing or communication models that do not reflect operational ground-station constraints. To explicitly model this intermittent information availability, we formulate the spacecraft-to-spacecraft collision avoidance problem as a semi-decentralized POMDP (SDec-POMDP), where we govern information propagation directly by realistic ground-station visibility windows. Joint maneuver policies are computed using approximate Recursive Small-Step Semi-Decentralized A* (RS-SDA*), following the state-of-the-art A*-based lineage for decentralized multiagent planning. Across a representative suite of conjunction scenarios, semi-decentralized planning recovers near-centralized maneuver quality while requiring 28.5% fewer synchronization events than continuous coordination. Comparisons with representative rule-based operator heuristics further show that communication-aware planning more consistently achieves the desired operational miss-distance band while minimizing unnecessary trajectory deviation. Together, these results establish a practical planning framework for autonomous collision avoidance under realistic intermittent communication, bridging the gap between idealized centralized coordination and fully decentralized planning execution.

==> Content/conjGeneration.tex <==
\section{A Parameterized Framework for Generating Physically Consistent Spacecraft Conjunction Benchmarks}

\section{Conjunction Scenario Generation}

\subsection{Motivation}

Representative conjunction benchmarks are essential for evaluating spacecraft collision avoidance algorithms. Existing datasets are typically derived either from historical conjunction events or from random sampling of orbital elements. Historical events provide operational realism but limited control over encounter geometry, while unconstrained orbital sampling often produces redundant or physically unrealistic conjunctions. For algorithm evaluation, it is desirable to generate conjunctions whose geometric properties can be varied systematically while maintaining physically realizable spacecraft orbits.

To address this need, we construct conjunctions by directly parameterizing the encounter at the predicted time of closest approach (TCA). Rather than sampling orbital elements and searching for conjunctions, the desired encounter geometry is specified first, after which the secondary spacecraft orbit is reconstructed subject to orbital feasibility constraints. This approach enables systematic coverage of the conjunction geometry space while producing reproducible benchmark scenarios.

\subsection{Encounter Parameterization}

Each conjunction is defined in the Radial--Transverse--Normal (RTN) frame of the primary spacecraft at TCA. The relative velocity vector is parameterized using spherical coordinates consisting of a velocity magnitude, a polar angle measured from the radial direction, and an azimuth angle within the transverse-normal plane. A miss vector is then prescribed in the plane perpendicular to the relative velocity vector such that

\begin{equation}
    \mathbf{r}_{miss}\cdot\mathbf{v}_{rel}=0,
\end{equation}

ensuring that the constructed encounter corresponds to a true closest approach where the relative separation rate is zero.

Although the complete encounter is represented in RTN coordinates, the collision avoidance model primarily depends on three quantities: the perpendicular separation

\begin{equation}
d_{\perp}=\sqrt{R^{2}+N^{2}},
\end{equation}

the along-track timing offset $\delta T_{0}$, and the relative along-track closing velocity. These quantities define an encounter angle

\begin{equation}
\theta=\tan^{-1}\left(\frac{d_{\perp}}{|\delta T_{0}|}\right),
\end{equation}

which naturally classifies conjunctions into head-on, oblique, and cross-track encounters.

\subsection{Physically Realizable Orbit Construction}

The primary spacecraft is fixed in a representative near-circular LEO reference orbit with

\begin{center}
$a \approx 6928$ km, \quad
$e = 0.001$, \quad
$i = 55^\circ$, \quad
$\Omega = 20^\circ$, \quad
$\omega = 0^\circ$, \quad
$M = 0^\circ$.
\end{center}

Given the desired encounter geometry, the secondary spacecraft orbit is reconstructed to satisfy the prescribed relative state at TCA. Plane-crossing encounters are generated using a closed-form construction relating relative velocity magnitude to the inclination difference,

\begin{equation}
v_{rel}=2v_{orb}\sin\left(\frac{\Delta i}{2}\right),
\end{equation}

which maintains near-circular secondary spacecraft orbits over a wide range of inclination differences, including retrograde encounters.

Each candidate orbit is required to satisfy basic LEO feasibility constraints, including a minimum perigee altitude of 150 km, maximum apogee altitude of 2000 km, and eccentricity less than 0.25. In practice, the generated benchmark scenarios remain nearly circular ($e\le0.005$), preserving the validity of the reduced collision geometry used throughout this work.

\subsection{Scenario Sampling}

Conjunctions are generated by sweeping the principal geometric parameters governing encounter behavior. The benchmark spans multiple screening miss distances, reference orbital altitudes, plane-crossing angles, and miss-vector orientations, producing broad coverage of representative collision geometries encountered in LEO.

Candidate conjunctions are grouped according to altitude, encounter angle, and plane-crossing geometry. A round-robin selection strategy is then applied to obtain approximately uniform coverage across the conjunction space while avoiding overrepresentation of any particular encounter class.

The benchmark presented in this work contains 52 representative conjunction scenarios spanning four screening miss distances (1, 2, 5, and 10 km), three altitude regimes (550, 800, and 1200 km), plane-crossing angles up to approximately $115^\circ$, and encounter angles ranging from approximately $3^\circ$ to $90^\circ$. Denser parameter sweeps containing several hundred to several thousand conjunctions were used during method development but are not included in the evaluation benchmark.

\subsection{Scenario Verification}

Every generated conjunction is independently verified using the Brahe astrodynamics library. A golden-section search over a $\pm600$ s interval surrounding the predicted TCA identifies the true minimum separation. Candidate conjunctions are retained only if the realized TCA differs from the constructed TCA by less than one second, the realized three-dimensional miss distance agrees with the prescribed miss distance within tolerance, and the encounter contains a single unique closest approach. Scenarios failing any verification criterion are discarded and regenerated.

For each accepted conjunction, the benchmark stores the reconstructed spacecraft orbital elements, verified closest-approach geometry, relative velocity vector expressed in RTN coordinates, and associated verification statistics to support reproducible evaluation and downstream analysis.

\begin{table}[t]
\centering
\caption{Parameter ranges used to generate the conjunction benchmark.}
\label{tab:generator_parameters}
\begin{tabular}{ll}
\toprule
Parameter & Values \\
\midrule
Reference altitude & 550, 800, \qty{1200}{\km}\\
Screening miss distance & 1, 2, 5, \qty{10}{\km}\\
Plane-crossing angle ($\Delta i$) & $0^\circ$--$115^\circ$ \\
Miss-vector rotation & $0^\circ$--$157.5^\circ$ (22.5$^\circ$ increments) \\
Encounter angle & $3^\circ$--$90^\circ$ \\
Reference orbit & Near-circular LEO ($e=0.001$) \\
Orbit feasibility & $150 \le h_p$, $h_a \le 2000$ km, $e \le 0.25$ \\
Verification & Brahe closest-approach validation \\
\bottomrule
\end{tabular}
\end{table}
